Graph-Theoretic Characterization of Noise Capacity of Conditional Disclosure of Secrets

In the Conditional Disclosure of Secrets (CDS) problem, Alice and Bob hold inputs $x\in \mathcal{X}$ and $y\in \mathcal{Y}$ and share a secret. Let $f:\mathcal{X}\times\mathcal{Y}\to\{0,1\}$ be a function such that the secret is revealed to a third party, Carol, if and only if $f(x,y)=1$. To protect the secret when $f(x,y)=0$, Alice and Bob share a common noise variable unknown to Carol. We study the \emph{noise capacity} of CDS, defined as the maximum number of secret bits that can be securely revealed per noise bit. We first derive necessary and sufficient conditions on $f$, represented by a CDS graph, for the extremal case where the noise capacity equals $1$. We then develop converse bounds on the noise rate for all linear schemes: $\frac{(\rho-1)(d-1)}{\rho d-1}$ if $\rho$ is finite, and $\frac{d-1}{d}$ if $\rho$ is infinite, where $\rho$ is the covering parameter of the CDS graph and $d$ is the number of unqualified edges in an unqualified path. Under maximal communication efficiency (message size equals secret size), we refine these bounds by analyzing qualified components and their connections. Achievability is shown for CDS instances with cyclic qualified edges and a single unqualified path. This graph-theoretic framework links noise efficiency limits to the unqualified path distance and covering parameter, providing a systematic method to analyze CDS under arbitrary graph topologies.

==> author_isit.tex <==
\author{\IEEEauthorblockN{Zhou Li\IEEEauthorrefmark{1}\IEEEauthorrefmark{3}, 
Siyan Qin\IEEEauthorrefmark{1}, 
Xiang Zhang\IEEEauthorrefmark{2},
Jihao Fan\IEEEauthorrefmark{3}\IEEEauthorrefmark{4}, 
Haiqiang Chen\IEEEauthorrefmark{1}, 
and Giuseppe Caire\IEEEauthorrefmark{2}
}
\IEEEauthorblockA{
Guangxi Key Laboratory of Multimedia Communications and Network Technology, Guangxi University\IEEEauthorrefmark{1}\\
Department of Electrical Engineering and Computer Science, Technical University of Berlin\IEEEauthorrefmark{2}\\
School of Cyber Science and Engineering, Nanjing University of Science and Technology\IEEEauthorrefmark{3}\\
Laboratory for Advanced Computing and Intelligence Engineering, 214083, Wuxi, China\IEEEauthorrefmark{4}\\
Email:~\IEEEauthorrefmark{1}\{lizhou, haiqiang\}@gxu.edu.cn, \IEEEauthorrefmark{1}2413302012@st.gxu.edu.cn, \IEEEauthorrefmark{2}\{xiang.zhang, caire\}@tu-berlin.de,\\
\IEEEauthorrefmark{3}jihao.fan@outlook.com,
}
}


















==> other/abstract_formal.tex <==
In the problem of Conditional Disclosure of Secrets (CDS), two  parties, Alice and Bob, each have an input and share a common secret. Their goal is to reveal the secret to a third party, Carol, as efficiently as possible, but only if their inputs meet certain functional criteria. To protect the secret, both Alice and Bob introduce noise. This work aims to determine the noise capacity, defined as the maximum number of secret bits that can be securely revealed per bit of total noise. We establish the necessary and sufficient conditions for achieving the extremal case where the CDS noise capacity is maximized at a value of \(1\). Beyond the best-case scenarios, we characterize the linear noise capacity and derive an upper bound for the linear noise rate applicable to all CDS instances. Specifically, this upper bound is \( (\rho-1)(d-1)/(\rho d-1)\), where  \(\rho \) is the covering parameter of the graph representation of \(f\), and  \(d\) is the number of unqualified edges in residing unqualified path.
